Efficiera Residual Networks: Hardware-Friendly Fully Binary Weight with 2-bit Activation Model Achieves Practical ImageNet Accuracy

The edge-device environment imposes severe resource limitations, encompassing computation costs, hardware resource usage, and energy consumption for deploying deep neural network models. Ultra-low-bit quantization and hardware accelerators have been explored as promising approaches to address these challenges. Ultra-low-bit quantization significantly reduces the model size and the computational cost. Despite progress so far, many competitive ultra-low-bit models still partially rely on float or non-ultra-low-bit quantized computation such as the input and output layer. We introduce Efficiera Residual Networks (ERNs), a model optimized for low-resource edge devices. ERNs achieve full ultra-low-bit quantization, with all weights, including the initial and output layers, being binary, and activations set at 2 bits. We introduce the shared constant scaling factor technique to enable integer-valued computation in residual connections, allowing our model to operate without float values until the final convolution layer. Demonstrating competitiveness, ERNs achieve an ImageNet top-1 accuracy of 72.5pt with a ResNet50-compatible architecture and 63.6pt with a model size less than 1MB. Moreover, ERNs exhibit impressive inference times, reaching 300FPS with the smallest model and 60FPS with the largest model on a cost-efficient FPGA device.

==> table/ablation.tex <==
\begin{table}[htbp]
\caption{The effect of inference scheme on ImageNet Top1 Accuracy of ERNs-18 and ERNs-50}
\label{tab:ablation}
\begin{center}
\begin{tabular}{l|rr}
\hline
Component & \multicolumn{1}{c}{ERNs-18}  & \multicolumn{1}{c}{ERNs-50} \\ \hline
- & 64.8 & 71.3  \\ \hline
w/o tencrop augmentation  & 62.2 (-2.6) & 69.5 (-1.8)\\ \hline
w/o increased resolution & 61.6 (-0.6) & 68.9 (-0.6)\\ \hline
\end{tabular}
\end{center}
\end{table}

